On Clustered Statistical MIMO Millimeter Wave Channel Simulation

The use of mmWave frequencies is one of the key strategies to achieve the fascinating 1000x increase in the capacity of future 5G wireless systems. While for traditional sub-6 GHz cellular frequencies several well-developed statistical channel models are available for system simulation, similar tools are not available for mmWave frequencies, thus preventing a fair comparison of independently developed transmission and reception schemes. In this paper we provide a simple albeit accurate statistical procedure for the generation of a clustered MIMO channel model operating at mmWaves, for both the cases of slowly and rapidly time-varying channels. Matlab scripts for channel generation are also provided, along with an example of their use.

==> abbreviations.tex <==

\renewcommand{\arraystretch}{1.5}
\newcommand{\spazio}{\rule[-6mm]{0mm}{0mm}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\wt}{\widetilde}
\newcommand{\ov}{\overline}
\newcommand{\LL}{{\cal L}}
\newcommand{\bN}{\mbox{\boldmath $N$}}
\newcommand{\br}{\mbox{\boldmath $r$}}
\newcommand{\bT}{\mbox{\boldmath $T$}}
\newcommand{\bJ}{\mbox{\boldmath $J$}}
\newcommand{\bs}{\mbox{\boldmath $s$}}
\newcommand{\uH}{\underline{H}}
\newcommand{\uh}{\underline{h}}
\newcommand{\bb}{\mbox{\boldmath $b$}}
\newcommand{\bbf}{\mbox{\boldmath $f$}}
\newcommand{\ba}{\mbox{\boldmath $a$}}
\newcommand{\bq}{\mbox{\boldmath $q$}}
\newcommand{\bp}{\mbox{\boldmath $p$}}
\newcommand{\be}{\mbox{\boldmath $e$}}
\newcommand{\bzero}{\mbox{\boldmath $0$}}
\newcommand{\bM}{\mbox{\boldmath $M$}}
\newcommand{\wi}{\widetilde}
\newcommand{\bDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\wh}{\widehat}
\newcommand{\bA}{\mbox{\boldmath $A$}}
\newcommand{\bP}{\mbox{\boldmath $P$}}
\newcommand{\bC}{\mbox{\boldmath $C$}}
\newcommand{\bX}{\mbox{\boldmath $X$}}
\newcommand{\bh}{\mbox{\boldmath $h$}}
\newcommand{\bH}{\mbox{\boldmath $H$}}
\newcommand{\bK}{\mbox{\boldmath $K$}}
\newcommand{\bk}{\mbox{\boldmath $k$}}
\newcommand{\bc}{\mbox{\boldmath $c$}}
\newcommand{\bS}{\mbox{\boldmath $S$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bZ}{\mbox{\boldmath $Z$}}
\newcommand{\bU}{\mbox{\boldmath $U$}}
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bB}{\mbox{\boldmath $B$}}
\newcommand{\bE}{\mbox{\boldmath $E$}}
\newcommand{\bV}{\mbox{\boldmath $V$}}
\newcommand{\bL}{\mbox{\boldmath $L$}}
\newcommand{\bG}{\mbox{\boldmath $G$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bW}{\mbox{\boldmath $W$}}
\newcommand{\bLambda}{{\bf \Lambda}}
\newcommand{\bpsi}{{\bf \psi}}
\newcommand{\bPsi}{{\bf \Psi}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bell}{\mbox{\boldmath $\ell$}}
%\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bi}{\mbox{\boldmath $i$}}
\newcommand{\bu}{\mbox{\boldmath $u$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\bdelta}{\mbox{\boldmath $\delta$}}
\newcommand{\bx}{\mbox{\boldmath $x$}}
\newcommand{\bz}{\mbox{\boldmath $z$}}
\newcommand{\bg}{\mbox{\boldmath $g$}}
\newcommand{\bn}{\mbox{\boldmath $n$}}
%\newcommand{\bm}{\mbox{\boldmath $m$}}
\newcommand{\bv}{\mbox{\boldmath $v$}}
\newcommand{\bd}{\mbox{\boldmath $d$}}
\newcommand{\bQ}{\mbox{\boldmath $Q$}}
\newcommand{\bO}{\mbox{\boldmath $O$}}
\newcommand{\bR}{\mbox{\boldmath $R$}}
\newcommand{\bF}{\mbox{\boldmath $F$}}
\newcommand{\bphi}{{\bf \Phi}}
\newcommand{\bI}{\mbox{\boldmath $I$}}
\newcommand{\bbtheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bbbeta}{\mbox{\boldmath $\eta$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\bSigma}{{\bf \Sigma}}
\newcommand{\bPi}{{\bf \Pi}}
\newcommand{\bOmega}{{\bf \Omega}}
\newcommand{\bt}{\mbox{\boldmath $t$}}
\newcommand{\bD}{\mbox{\boldmath $D$}}
\newcommand{\by}{\mbox{\boldmath $y$}}
\newcommand{\ds}{\displaystyle}
\newcommand{\bw}{\mbox{\boldmath $w$}}
\newcommand{\bY}{\mbox{\boldmath $Y$}}
\newcommand{\K}{{\cal K}}
\newcommand{\G}{{\cal G}}
\newcommand{\N}{{\cal N}_0}
\hyphenation{E-let-tro-ni-ca}
\newcommand{\bbeta}{\mbox{\boldmath{$\beta$}}}
\def\M{{\cal M}}
\def\R{{\cal R}}
\def\S{{\cal S}}
\def\I{{\cal I}}
\newcommand{\beq}{\begin{equation}}

% Set of real, integer, etc., numbers, l_2 spaces, real, and imaginary parts
\newcommand{\Reals}    {{\mathbb R}} % {{{\mathrm I\!R}}}  
\newcommand{\Cplx}      {{{\mathsf I}\!\!\!{\mathrm C}}} %{{\mathbb C}}
\newcommand{\NCplx}     {{{\mathcal{CN}}}} % Complex normal distribution
\newcommand{\Ints}      {{{\mathbb Z}}} % Z set of all integers
\newcommand{\Rats}      {{{\mathsf I}\!\!\!{\mathrm Q}}}    % Q set of all rational numbers
\newcommand{\Nats}      {{{\mathrm{ I\!N}}}} % N set of all natural numbers
\newcommand{\Tee}{      {{\mathbb T}}}
\newcommand{\ltwo}      {{\ell_2}}
\newcommand{\lone}      {{\ell_1}}
\newcommand{\Ltwo}      {{\mathbb L}^2}
\newcommand{\LtR}       {\Ltwo(\Reals)}
\newcommand{\Real}[1]   {{\mathrm{Re}\left\{#1\right\}}}
\newcommand{\Imag}[1]   {{\mathrm{Im}\left\{#1\right\}}}
\newcommand{\real}      {{\mathcal{R}} e}
\newcommand{\imag}      {{\mathcal{I}} m}



% Some commands for nice typesetting
\newcommand{\ie}        {i.~e., \hspace{2pt}}      % id est
\newcommand{\eg}        {e.~g., \hspace{2pt}}      %
\newcommand{\define}    {\stackrel{\triangle}{=}}  % define, an '=' with an '^' on top
\newcommand{\D}  {^{\dag}}               % Dagger, includes '^' !
\newcommand{\T}  {{\mathsf{T}}}          % Transpose, no '^' !
\newcommand{\ct} {{\mathsf{*}}}          % conjugate complex, should use \dag for conjugate complex transpose
\newcommand{\half}{{{^1\!\!\scriptscriptstyle{/}\!}_2}}       % a nice 1/2
\newcommand{\mrsss}[1]   {{\mathrm{\scriptscriptstyle{#1}}}}  % math roman scriptscriptstyle - works well for sub and superscripts
\newcommand{\sth}     {{\mathrm{th}}}    % superscript th \th is already defined -- the $k^\sth$ user
\newcommand{\diag}    {{\mathrm{diag}}}  % for diag{1, 2, 3}
\newcommand{\tr}      {{\mathrm{tr}}}    % trace of a matrix
\newcommand{\Res}     {{\mathrm{Res}}}   % Residue
\newcommand{\ld}      {{\mathrm{ld}}}    % logarithmus dualis
\newcommand{\barg}    {\overline{\gamma}}     % average received SNR
\newcommand{\sqgb}    {\sqrt{\barg}}     % square root of the average received SNR
\newcommand{\e}       {{\mathrm e}}      % e for exponential function
\newcommand{\E}       {{\mathrm E}}      % Expectation
\newcommand{\lNZ}     {{\lambda_{\mathsf{NZ}}}} % to denote the non-zero eigenvalues of a matrix
\newcommand{\Mt}      {{M_{\!\mrsss{T}}}}% N_T no of transmit antennas
\newcommand{\Mr}      {{M_{\!\mrsss{R}}}}% N_R no of receive antennas
\newcommand{\uple}    {{\mathrm{ul}}}    % upper-left
\newcommand{\upri}    {{\mathrm{ur}}}    % upper-right
\newcommand{\lole}    {{\mathrm{ll}}}    % lower-left
\newcommand{\lori}    {{\mathrm{lr}}}    % lower-right

% Bold numbers
\newcommand{\Zrb}     {{\mathbf 0}}      % bold zero
\newcommand{\Oneb}    {{\mathbf 1}}      % bold one

% Define bold roman letters
\newcommand{\ab}{{\mathbf a}}  \newcommand{\Ab}{{\mathbf A}}
\newcommand{\cb}{{\mathbf c}}  \newcommand{\Cb}{{\mathbf C}}
\newcommand{\db}{{\mathbf d}}  \newcommand{\Db}{{\mathbf D}}
\newcommand{\eb}{{\mathbf e}}  \newcommand{\Eb}{{\mathbf E}}
\newcommand{\fb}{{\mathbf f}}  \newcommand{\Fb}{{\mathbf F}}
\newcommand{\gb}{{\mathbf g}}  \newcommand{\Gb}{{\mathbf G}}
\newcommand{\hb}{{\mathbf h}}  \newcommand{\Hb}{{\mathbf H}}
\newcommand{\ib}{{\mathbf i}}  \newcommand{\Ib}{{\mathbf I}}
\newcommand{\jb}{{\mathbf j}}  \newcommand{\Jb}{{\mathbf J}}
\newcommand{\kb}{{\mathbf k}}  \newcommand{\Kb}{{\mathbf K}}
\newcommand{\lb}{{\mathbf l}}  \newcommand{\Lb}{{\mathbf L}}
\newcommand{\mb}{{\mathbf m}}  \newcommand{\Mb}{{\mathbf M}}
\newcommand{\nb}{{\mathbf n}}  \newcommand{\Nb}{{\mathbf N}}
\newcommand{\ob}{{\mathbf o}}  \newcommand{\Ob}{{\mathbf O}}
\newcommand{\pb}{{\mathbf p}}  \newcommand{\Pb}{{\mathbf P}}
\newcommand{\qb}{{\mathbf q}}  \newcommand{\Qb}{{\mathbf Q}}
\newcommand{\rb}{{\mathbf r}}  \newcommand{\Rb}{{\mathbf R}}
\renewcommand{\sb}{{\mathbf s}}\newcommand{\Sb}{{\mathbf S}} %\sb is equiv. to _ in Tex, unnecessary.
\newcommand{\tb}{{\mathbf t}}  \newcommand{\Tb}{{\mathbf T}}
\newcommand{\ub}{{\mathbf u}}  \newcommand{\Ub}{{\mathbf U}}
\newcommand{\vb}{{\mathbf v}}  \newcommand{\Vb}{{\mathbf V}}
\newcommand{\wb}{{\mathbf w}}  \newcommand{\Wb}{{\mathbf W}}
\newcommand{\xb}{{\mathbf x}}  \newcommand{\Xb}{{\mathbf X}}
\newcommand{\yb}{{\mathbf y}}  \newcommand{\Yb}{{\mathbf Y}}
\newcommand{\zb}{{\mathbf z}}  \newcommand{\Zb}{{\mathbf Z}}

% Define bold greek letters, lower and upper case
\newcommand{\alphab}      {{\bm \alpha}}          \newcommand{\Alphab}   {{\mathbf {\mathrm A}}}
\newcommand{\betab}       {{\bm \beta}}           \newcommand{\Betab}    {{\mathbf {\mathrm B}}}
\newcommand{\gammab}      {{\bm \gamma}}          \newcommand{\Gammab}   {{\bm \Gamma}}
\newcommand{\deltab}      {{\bm \delta}}          \newcommand{\Deltab}   {{\bm \Delta}}
\newcommand{\epsilonb}    {{\bm \epsilon}}        \newcommand{\Epsilonb} {{\mathbf {\mathrm E}}}
\newcommand{\varepsilonb} {{\bm \varepsilon}}
\newcommand{\vepsilonb}   {{\bm \varepsilon}}
\newcommand{\zetab}       {{\bm \zeta}}           \newcommand{\Zetab}    {{\mathbf {\mathrm Z}}}
\newcommand{\etab}        {{\bm \eta}}            \newcommand{\Etab}     {{\mathbf {\mathrm H}}}
\newcommand{\thetab}      {{\bm \theta}}          \newcommand{\Thetab}   {{\bm \Theta}}
\newcommand{\varthetab}   {{\bm \vartheta}}
\newcommand{\vthetab}     {{\bm \vartheta}}
\newcommand{\iotab}       {{\bm \iota}}           \newcommand{\Iotab}    {{\mathbf {\mathrm I}}}
\newcommand{\kappab}      {{\bm \kappa}}          \newcommand{\Kappab}   {{\mathbf {\mathrm K}}}
\newcommand{\lambdab}     {{\bm \lambda}}         \newcommand{\Lambdab}  {{\bm \Lambda}}
\newcommand{\mub}         {{\bm \mu}}             \newcommand{\Mub}      {{\mathbf {\mathrm M}}}
\newcommand{\nub}         {{\bm \nu}}             \newcommand{\Nub}     	{{\mathbf {\mathrm N}}}	
\newcommand{\xib}         {{\bm \xi}}             \newcommand{\Xib}      {{\bm \Xi}}
\newcommand{\omicronb}    {{\mathbf {\mathrm o}}} \newcommand{\Omicronb} {{\mathbf {\mathrm O}}}
\newcommand{\pib}         {{\bm \pi}}             \newcommand{\Pib}      {{\bm \Pi}}
\newcommand{\varpib}      {{\bm \varpi}}
\newcommand{\vpib}        {{\bm \varpi}}
\newcommand{\rhob}        {{\bm \rho}}            \newcommand{\Rhob}     {{\mathbf {\mathrm P}}}
\newcommand{\varrhob}     {{\bm \varrho}}
\newcommand{\vrhob}       {{\bm \varrho}}
\newcommand{\sigmab}      {{\bm \sigma}}          \newcommand{\Sigmab}   {{\bm \Sigma}}
\newcommand{\varsigmab}   {{\bm \varsigma}}
\newcommand{\vsigmab}     {{\bm \varsigma}}
\newcommand{\taub}        {{\bm \tau}}            \newcommand{\Taub}     {{\mathbf {\mathrm T}}}
\newcommand{\upsilonb}    {{\bm \upsilon}}        \newcommand{\Upsilonb} {{\bm \Upsilon}}
\newcommand{\phib}        {{\bm \phi}}            \newcommand{\Phib}     {{\bm \Phi}}
\newcommand{\varphib}     {{\bm \varphi}}
\newcommand{\vphib}       {{\bm \varphi}}
\newcommand{\chib}        {{\bm \chi}}            \newcommand{\Chib}     {{\mathbf {\mathrm X}}}
\newcommand{\psib}        {{\bm \psi}}            \newcommand{\Psib}     {{\bm \Psi}}
\newcommand{\omegab}      {{\bm \omega}}          \newcommand{\Omegab}   {{\bm \Omega}}

% Calligraphic letters, normal and bold
\newcommand{\Ac} {{\mathcal A}}         \newcommand{\Ak} {{\bm {\mathcal A}}}
\newcommand{\Bc} {{\mathcal B}}         \newcommand{\Bk} {{\bm {\mathcal B}}}
\newcommand{\Cc} {{\mathcal C}}         \newcommand{\Ck} {{\bm {\mathcal C}}}
\newcommand{\Dc} {{\mathcal D}}         \newcommand{\Dk} {{\bm {\mathcal D}}}
\newcommand{\Ec} {{\mathcal E}}         \newcommand{\Ek} {{\bm {\mathcal E}}}
\newcommand{\Fc} {{\mathcal F}}         \newcommand{\Fk} {{\bm {\mathcal F}}}
\newcommand{\Gc} {{\mathcal G}}         \newcommand{\Gk} {{\bm {\mathcal G}}}
\newcommand{\Hc} {{\mathcal H}}         \newcommand{\Hk} {{\bm {\mathcal H}}}
\newcommand{\Ic} {{\mathcal I}}         \newcommand{\Ik} {{\bm {\mathcal I}}}
\newcommand{\Jc} {{\mathcal J}}         \newcommand{\Jk} {{\bm {\mathcal J}}}
\newcommand{\Kc} {{\mathcal K}}         \newcommand{\Kk} {{\bm {\mathcal K}}}
\newcommand{\Lc} {{\mathcal L}}         \newcommand{\Lk} {{\bm {\mathcal L}}}
\newcommand{\Mc} {{\mathcal M}}         \newcommand{\Mk} {{\bm {\mathcal M}}}
\newcommand{\Nc} {{\mathcal N}}         \newcommand{\Nk} {{\bm {\mathcal N}}}
\newcommand{\Oc} {{\mathcal O}}         \newcommand{\Ok} {{\bm {\mathcal O}}}
\newcommand{\Pc} {{\mathcal P}}         \newcommand{\Pk} {{\bm {\mathcal P}}}
\newcommand{\Qc} {{\mathcal Q}}         \newcommand{\Qk} {{\bm {\mathcal Q}}}
\newcommand{\Rc} {{\mathcal R}}         \newcommand{\Rk} {{\bm {\mathcal R}}}
\newcommand{\Sc} {{\mathcal S}}         \newcommand{\Sk} {{\bm {\mathcal S}}}
\newcommand{\Tc} {{\mathcal T}}         \newcommand{\Tk} {{\bm {\mathcal T}}}
\newcommand{\Uc} {{\mathcal U}}         \newcommand{\Uk} {{\bm {\mathcal U}}}
\newcommand{\Vc} {{\mathcal V}}         \newcommand{\Vk} {{\bm {\mathcal V}}}
\newcommand{\Wc} {{\mathcal W}}         \newcommand{\Wk} {{\bm {\mathcal W}}}
\newcommand{\Xc} {{\mathcal X}}         \newcommand{\Xk} {{\bm {\mathcal X}}}
\newcommand{\Yc} {{\mathcal Y}}         \newcommand{\Yk} {{\bm {\mathcal Y}}}
\newcommand{\Zc} {{\mathcal Z}}         \newcommand{\Zk} {{\bm {\mathcal Z}}}


\newcommand{\Grb}   {{\mathbf {\mathrm V}}}

\newcommand{\Qulk} {{\underline{{\bm {\mathcal Q}}}}}

\newcommand{\Gulc} {{\underline{\mathcal G}}}
\newcommand{\Culc} {{\underline{\mathcal C}}}

% underlined upper and lower case letters
\newcommand{\Aul}  {{\underline A}}              \newcommand{\aul}  {{\underline a}}
\newcommand{\Bul}  {{\underline B}}              \newcommand{\bul}  {{\underline b}}
\newcommand{\Cul}  {{\underline C}}              \newcommand{\cul}  {{\underline c}}
\newcommand{\Dul}  {{\underline D}}              \newcommand{\dul}  {{\underline d}}
\newcommand{\Eul}  {{\underline E}}              \newcommand{\eul}  {{\underline e}}
\newcommand{\Ful}  {{\underline F}}              \newcommand{\ful}  {{\underline f}}
\newcommand{\Gul}  {{\underline G}}              \newcommand{\gul}  {{\underline g}}
\newcommand{\Hul}  {{\underline H}}              \newcommand{\hul}  {{\underline h}}
\newcommand{\Iul}  {{\underline I}}              \newcommand{\iul}  {{\underline i}}
\newcommand{\Jul}  {{\underline J}}              \newcommand{\jul}  {{\underline j}}
\newcommand{\Kul}  {{\underline K}}              \newcommand{\kul}  {{\underline k}}
\newcommand{\Lul}  {{\underline L}}              \newcommand{\lul}  {{\underline l}}
\newcommand{\Mul}  {{\underline M}}              \newcommand{\mull} {{\underline m}}
\newcommand{\Nul}  {{\underline N}}              \newcommand{\nul}  {{\underline n}}
\newcommand{\Oul}  {{\underline 0}}              \newcommand{\oul}  {{\underline o}}
\newcommand{\Pul}  {{\underline P}}              \newcommand{\pul}  {{\underline p}}
\newcommand{\Qul}  {{\underline Q}}              \newcommand{\qul}  {{\underline q}}
\newcommand{\Rul}  {{\underline R}}              \newcommand{\rul}  {{\underline r}}
\newcommand{\Sul}  {{\underline S}}              \newcommand{\sul}  {{\underline s}}
\newcommand{\Tul}  {{\underline T}}              \newcommand{\tul}  {{\underline t}}
\newcommand{\Uul}  {{\underline U}}              \newcommand{\uul}  {{\underline u}}
\newcommand{\Vul}  {{\underline V}}              \newcommand{\vul}  {{\underline v}}
\newcommand{\Wul}  {{\underline W}}              \newcommand{\wul}  {{\underline w}}
\newcommand{\Xul}  {{\underline X}}              \newcommand{\xul}  {{\underline x}}
\newcommand{\Yul}  {{\underline Y}}              \newcommand{\yul}  {{\underline y}}
\newcommand{\Zul}  {{\underline Z}}              \newcommand{\zul}  {{\underline z}}

% Misc. short-cuts
\newcommand{\mc}[1]     {{\mathcal{#1}}}        % mathcal
\newcommand{\what}[1]   {\widehat{#1}}          % widehat
\newcommand{\wtld}[1]   {\widetilde{#1}}        % widetilde
\newcommand{\Portho}[1] {\Pb_{#1}^{\perp}}      % orthogonal projection


\newcounter{MYtempeqncnt}
\setlength\arraycolsep{2pt} \sloppy

\newcommand{\threshold}{\mbox{$
\begin{array}{c} \stackrel{\textstyle H_1}{\textstyle>}\\
\stackrel{\textstyle <}{\textstyle H_0}
\end{array}$}}
\newcommand{\nchoosek}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
\newcommand{\gammabar}{\bar{\gamma}}
\newcommand{\Prob}{\mbox{Prob}}

\def\QED{\mbox{\rule[0pt]{1.5ex}{1.5ex}}}
\setlength\arraycolsep{2pt} \sloppy

\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
%\newtheorem{algorithm}{Algorithm}
%\newtheorem{proof}{Proof}

\def\IR{{\mathbb R}}
\def\IC{{\mathbb C}}


==> acronyms.tex <==
\makeglossaries

\newacronym{mac}{MAC}{multiple-access channel}
\newacronym{bc}{BC}{broadcast channel}
\newacronym{mimo}{MIMO}{multiple-input multiple-output}
\newacronym{comp}{CoMP}{cooperative multi-point}
\newacronym{siso}{SISO}{single-input single-output}
\newacronym{af}{AF}{amplify-and-forward}
\newacronym{df}{DF}{decode-and-forward}
\newacronym{cf}{CF}{compress-and-forward}
\newacronym{mwrc}{MWRC}{multi-way relay channel}
\newacronym{pde}{PDE}{partial data exchange}
\newacronym{fde}{FDE}{full data exchange}
\newacronym{iid}{i.i.d.\@}{independent and identically distributed}
\newacronym{awgn}{AWGN}{additive white Gaussian noise}
\newacronym{awg}{AWG}{additive white Gaussian}
\newacronym{sic}{SIC}{successive interference cancellation}
\newacronym{uwb}{UWB}{ultrawideband}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{sinr}{SINR}{signal-to-interference-plus-noise-ratio}
\newacronym{zf}{ZF}{zero-forcing}
\newacronym{mmse}{MMSE}{minimum mean square error}
\newacronym{sud}{SUD}{single user decoding}
\newacronym{dof}{DoF}{degrees of freedom}
\newacronym{gdof}{GDoF}{generalized degrees of freedom}
\newacronym{nnc}{NNC}{noisy network coding}
\newacronym{dmn}{DMN}{discrete memoryless network}
\newacronym{csi}{CSI}{channel state information}
\newacronym{ict}{ICT}{information and communications technology}
\newacronym{ee}{EE}{energy efficiency}
\newacronym{kkt}{KKT}{Karush-Kuhn-Tucker}
\newacronym{gee}{GEE}{global energy efficiency}
\newacronym{ian}{IAN}{treating interference as noise}
\newacronym{snd}{SND}{simultaneous non-unique decoding}
\newacronym{gnep}{GNEP}{Generalized Nash Equilibrium Problem}
\newacronym{nep}{NEP}{Generalized Nash Equilibrium Problem}
\newacronym{rhs}{RHS}{right-hand side}
\newacronym{lhs}{LHS}{left-hand side}
\newacronym{ofdma}{OFDMA}{orthogonal frequency division multiple access}
\newacronym{qos}{QoS}{quality-of-service}
\newacronym{d2d}{D2D}{device-to-device}

%	\newacronym{CDF}{cumulative distribution function}
%	\newacronym{PDF}{probability density function}
%	\newacronym{iid}{i.i.d.\@}{independent and identically distributed}
%	\newacronym{iff}{if and only if}

